Generalized affine buildings

In the present thesis geometric properties of non-discrete affine buildings are studied. We cover in particular affine $\Lambda$-buildings, which were introduced by Curtis Bennett in 1990 and which already have proven to be useful for applications. The main results are as follow: First we prove an extension theorem for ecological isomorphisms of buildings at infinity. Further, complementing a joint project with L. Kramer and R. Weiss, we give an algebraic proof of the existence of (necessarily) non-discrete affine buildings having Suzuki-Ree buildings at infinity. Most of the effort is put in the generalization of Kostant's convexity theorem for symmetric spaces in the setting of simplicial affine and affine $\Lambda$-buildings. The proofs are based on connections to representation theory as well as on methods borrowed from metric geometry.

==> files/a04conditionFC-alt.tex <==
\section{Finite covering conditions}\label{Sec_FC}

In section \ref{Sec_convexityRevisited} we made use of the \emph{finite cover condition} (FC) to prove that certain retractions are distance non-increasing. By the time this thesis was handed in, the proof that this condition holds for all generalized affine buildings in the sense of definition \ref{Def_LambdaBuilding} was not yet completed.
In the meantime I was able to verify (FC). Continue reading and you will find a proof on the subsequent pages.

We first prove a local version of the covering condition. Let in the following $(X,\App)$ be a generalized affine building. 

\begin{lemma}
Given an apartment $A$ and a point $z$ in $X$. Then $A$ is contained in the (finite) union of all Weyl chambers based at $z$ with equivalence class contained in $\partial A$.
\end{lemma}
\begin{proof}
Is $z$ contained in $A$ this is obvious. Hence assume that $z$ is not contained in $A$. Fix a point $p\in A$. By definition there exists an apartment $A'$ conatining $z$ and $p$. Let $S_+$ be a Weyl chamber based at $p$ containing $z$ and denote by $\sigma_+$ its germ at $p$. Theren there exists a unique Weylchamber $S_-$ contained in $A$ and based at $p$ such that its germ $\sigma_-$ is opposite $\sigma_+$ in the residue $\Delta_pX$. By Corollary~\ref{Cor_CO} the Weyl chambers $S_-$ and $S_+$ are contained in common apartment $A''$. Let $T$ be the unique representative of $\partial S_-$ which is based at $z$. Since $z\in S_+$ and $\sigma_+$ and $\sigma_-$ are opposite in $\Delta_pX$, the point $p$ is contained in $T$. Therefore $T$ contains $p$ and $\partial T$ is contained in $A$. Since there are only finitely many chambers in $\partial A$, and since for each of them there exists a unique representing Weyl chamber based at $z$, Corollary~\ref{Cor_WeylChamber} implies the assertion.
\end{proof}

\begin{lemma}\label{Lem_FC'}
Let $(X,\App)$ be an generalized affine building, let $x,y$ be points in $X$ contained in a common apartment $A$. For any $z\in X$ the following is true:
\begin{itemize}[label={(FC')}, leftmargin=*]
  \item[$\mathrm{(FC')}$] The segment $\seg_{A}(x,y)$ of $x$ and $y$ in $A$ is contained in a finite union of Weyl chambers based at $z$.
\end{itemize}
Furthermore, is $\mu$ a germ of a Weyl chamber based at $z$, then $\seg_{A}(x,y)$ is contained in a finite union of apartments containing $\mu$.
\end{lemma}
\begin{proof}
Condition (FC') is a direct consequence of the previous lemma.

Let $T$ be a Weyl chamber based at $z$, containing a given point $p\in \seg_A(x,y)$ with the property that $\partial T\in\partial A$. Apply Proposition~\ref{Prop_tec16} to $c\define\partial T$ and any Weyl chamber $S$ having germ  $\mu$ to obtain that $\seg_{A}(x,y)$ is contained in a finite union of apartments containing $\mu$.
\end{proof}

\begin{prop}\label{Prop_retraction}
For any apartment $A$ and any Weyl chamber $S$ in $X$ with germ in $A$ the retraction $r_{A,S}$, as defined in \ref{Def_vertexRetraction}, is distance non-increasing.
\end{prop}
\begin{proof}
Given two points $x$ and $y$ in $X$. By Proposition \ref{Lem_FC'} there exists a finite collection of apartments $A_0,\ldots, A_n$ enumerated and chosen in such a way that 
\begin{itemize}
  \item each $A_i$ contains the germ of $S$
  \item their union contains the segment of $x$ and $y$ in an apartment $A\ni x,y$ and 
  \item $A_i\cap A_{i+1} \neq \emptyset$ for all $i=0,\ldots, n-1$. 
\end{itemize}
Observe that one can find a finite sequence of points $x_i$, $i=0,\ldots,n$ with $x_0=0$ and $x_n=y$ such that 
$$d(x,y)=\sum_{i=0}^{n-1} d(x_i,x_{i+1})$$ and the points $x_i$ and $x_{i+1}$ are contained in $A_i$.

Notice that for all $i$ the restriction of $r_{A,S}$ to $A_i$ is an isomorphism onto $A$. Hence $d(x_i, x_{i+1})=d(\rho(x_i), \rho(x_{i+1}))$ for all $i\neq N$. By the triangle inequality for $d$ we have that $d(r(x),r(y))\leq d(x,y)$.
\end{proof}

Backtracking the proof of \ref{Prop_retraction} it is easy to see, that besides axioms $(A1)-(A4)$ and $(A6)$ we only needed the fact that the distance function on $X$, induced by the distance function on the model space which was defined in Section \ref{Sec_modelSpace}, satisfies the triangle inequality. From this we can define a distance non-increasing retraction satisfying the condition of $(A5)$. Therefore we have the following

\begin{corollary}
Let $(X,\App)$ be a space satisfying all conditions of Definition~\ref{Def_LambdaBuilding} except axiom $(A5)$. Then the following are equivalent:
\begin{itemize}[label={(A5*)}, leftmargin=*]
\item[(A5)] For any apartment $A$ and all $x\in A$ there exists a \emph{retraction} $r_{A,x}:X\to A$ such that $r_{A,x}$ does not increase distances and $r^{-1}_{A,x}(x)=\{x\}$.
\item[(A5')] The distance function $d$ on $X$, which is induced by the distance function on the model space, satisfies the triangle inequality.
\end{itemize}
\end{corollary}

Recall the definition of the \emph{segment} of point $x$ and $y$ in $X$:
$$\seg(x,y)\define\{z\in X : d(x,y)=d(x,z)+d(z,y) \}.$$

\begin{lemma}\label{Lem_tec31}
Let $x,y$ be points in $X$. Let $A$ be an apartment containing $x$ and $y$. For all retractions $r\define r_{A,S}$ based at a germ of a Weyl chamber $S$ in $A$ and all $z\in \seg(x,y)$ the following holds
\begin{enumerate}
  \item $r(z)\in \seg_A(x,y)$ and 
  \item $d(x,z)=d(x,r(z))$ as well as $d(y,z)=d(y,r(z))$.
\end{enumerate}
\end{lemma}
\begin{proof}
Since $r$ is distance non-increasing and $d$ satisfies the triangle inequality we have
$$
d(x,y)\leq d(x,r(z)) + d(y,r(z)) \leq d(x,z)+d(y,z)=d(x,y)
$$
and $r(z)$ is contained in $\seg_A(x,y)$.

Therefore 
\begin{equation}\label{Equ_1}
d(x,r(z))+d(r(z),y) = d(x,z)+d(z,y).
\end{equation}
The assumption $d(x,r(z)) < d(x,z)$ contradicts equation \ref{Equ_1}, hence $d(x,z)=d(x,r(z))$ and for symmetric reasons $d(y,z)=d(y,r(z))$.
\end{proof}


\begin{prop}
Segments are contained in apartments.
\end{prop}
\begin{proof}
Fix two points $x,y\in X$. Let $A$ be an apartment containing $x$ and $y$ and assume there exists $z\in\seg(x,y)\setminus A$.
Let $p$ be a point in $A$ such that there exists a Weyl chamber $S$ at $p$ containing $z$ whose intersection with $A$ equals $p$, i.e. the germ of $S$ is not contained in $A$. There are two different Weyl chambers $S_1$ and $S_2$ in $A$ with $\sigma_i\define \Delta_pS_i$ is opposite $\Delta_pS$ for $i=1,2$. Denote by $r_i$ the retraction $r_{A,S_i}$ onto $A$ based at the germ of $S_i$ and denote by $z_i$ the image of $z$ under $r_i$. Obviously $z_1\neq z_2$.

There exists a $w\in\sW$ such that $S_2=wS_1$ and $w.z_1 = z_2$. We therefore can find a sequence of reflections $r^i\define r_{\alpha_i, k_i}$, $i=1,\ldots, l$, with $\alpha_i\in B$ and $k_i\in\Lambda$ such that 
$$z_2= r^l(r^{l-1}( \ldots r^1(z_1) \ldots )).$$

But recall, that by Lemma \ref{Lem_segment} the segment of $x$ and $y$ in $A$ is the same as the convex hull of $x$ and $y$. Therefore $\seg_A(x,y)$ is contained in a Weyl chamber based at $x$.  By Lemma \ref{Lem_tec21} both $z_1$ and $z_2$ are contained in $\seg_A(x,y)$, therefore $w$ has to be the identity. But this contradicts the fact that $S_1\neq S_2$.
\end{proof}






